Data Pyramid for Embodied Manipulation: A Survey

Multimodal foundation models learned to see and to speak by consuming the whole internet. Embodied agents admit no such shortcut, since they require data that couple observations with physical states and actions. These signals can be provided, to varying degrees, by multiple data sources. In this work, we organize the embodied data ecosystem as a "pyramid'' spanning five complementary sources: real-robot data, UMI-style data, egocentric and exocentric data, simulation data, and general vision-language data. We organize the pyramid around the tension between scalability and robot alignment, and further characterize each source in terms of data quality, diversity, reusability, and physical fidelity. We then analyze recent embodied foundation models through the lens of data recipes, examining how different sources are selected, aligned, and mixed during pretraining. For embodied brain models, vision-language-action models, and world-action models alike, we relate data composition to capabilities in perception, reasoning, planning, action generation, and world prediction. To facilitate community use, we additionally consolidate over 10,000 hours of trajectories from widely used robot datasets into a unified LeRobot format, with transparent frame-level quality annotations for filtering. We close by discussing six open challenges: building large-scale tactile datasets, collecting failure and recovery data, developing scalable data-collection pipelines, aligning actions across embodiments, leveraging egocentric data for dexterous manipulation, and designing principled data recipes for robot learning. We hope this work lays the foundation for the design of next-generation embodied systems.

==> section/RealRobotData.bak.tex <==
\section{Real-Robot Data}


\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures_new/fig5.pdf}
    \vspace{-0.55cm}
    \caption{Overview of UMI data and real-robot data. \textbf{Left}: UMI data are collected with portable human-operated interfaces, emphasizing robot-free in-the-wild demonstrations, multimodal sensing, and relative end-effector trajectories. \textbf{Right}: real-robot data are collected on physical robot embodiments with diverse teleoperation systems, sensing modalities, and collection paradigms. Retargeting connects the two by transferring UMI demonstrations to executable robot actions for cross-embodiment deployment.}
    \label{fig:umi_real_robot}
\end{figure}


\subsection{Data Overview}

Real-robot data occupies the apex of the embodied-intelligence data pyramid, representing the layer closest to real-world execution. It is collected through the physical interaction between a robot and the environment, typically comprising sensory observations, robot states, and control actions. In contrast to human videos or embodiment-agnostic demonstration data, it directly captures the closed-loop relationship between perception, action, and physical consequences under a specific robotic embodiment. Consequently, it is characterized by high quality, physical fidelity, diversity, and reusability, making it the most direct source of supervision for learning executable manipulation policies and grounding model predictions in real-world dynamics.

The development of real-robot datasets has evolved from isolated, task-specific collections toward increasingly general and reusable data resources, as shown in Table~\ref{tab:real-robot-datasets}. Early efforts primarily focused on large numbers of trials for a small set of behaviors, such as robotic grasping, often collected using scripted controllers in controlled environments~\cite{pinto2016supersizing,kalashnikov2018scalable}. Subsequent datasets expanded toward human-operated demonstrations covering broader task sets and more diverse scenes~\cite{sharma2018multiple,mandlekar2018roboturk,ebert2021bridge,khazatsky2024droid}. More recent efforts further scale data collection across institutions, robot platforms, and application domains~\cite{o2024open,robomind2025,wu2025robocoin,hou2025robomind}, incorporating bimanual systems~\cite{agibotworld2026,fourier2025actionnet}, mobile manipulators~\cite{fu2024mobile}, humanoids~\cite{zhao2025humanoid,unitree2026unifolm}, and dexterous hands~\cite{zhang2026dexora,li2026deco}. This progression reflects a broader shift from collecting data for individual policies toward constructing large-scale data ecosystems for training generalist robot models.

Alongside this scaling trend, a complementary line of work specializes real-robot collection toward interaction regimes that generic household datasets underrepresent. PRISM~\cite{yu2026prism} targets high-precision, contact-rich industrial operations, recording more than 5,000 teleoperated trajectories over 25 manipulation tasks with synchronized multi-view RGB-D, force/torque, tactile, and robot-state measurements. SoftVTBench~\cite{jing2026softvtbench} instead focuses on deformable objects, pairing multi-view RGB, dual-finger tactile images and marker motion, proprioception, and language with evaluator-only finite-element states, so that physical interaction quality can be assessed independently of task success. A third direction adds structure rather than trajectories: RoboInter1.5~\cite{wang2026robointer15} re-annotates over 230K manipulation episodes with more than ten types of dense per-frame intermediate representations, including subtasks, primitive skills, object and gripper grounding, affordance, grasp poses, contact points, and motion traces. Together these efforts suggest that the marginal value of new real-robot data increasingly lies in covering underrepresented contact regimes and in enriching annotation depth, rather than in raw trajectory count alone.

Annotation enrichment can also improve the geometric value of existing demonstrations. DROID-3D~\cite{bardhan2026depthworld} augments over 70,000 DROID episodes with learned stereo depth and robot-grounded multi-view calibration, jointly optimizing shared robot parameters and scene-specific extrinsics. These annotations support RGB-depth prediction in DepthWorld, but the depth remains estimated and the held-out-trajectory evaluation uses the same robots and laboratories as training. The contribution therefore expands supervision quality rather than the number of independently collected physical interactions. Temporal enrichment can instead use the robot state stream: KiRoSe~\cite{xie2026kirose} learns transition-supervised sparse motion tokens and uses a language model to segment kinematic trajectories, retaining the need for annotated training transitions. FLORA~\cite{leng2026flora} complements this approach with models for timestamped captions and outcome or process reward labels, supplying semantic supervision for filtering and post-training rather than additional physical trajectories.

GazeAct~\cite{pani2026gazeact} enriches real-robot demonstrations with the teleoperator's gaze on the robot-camera display, synchronizing attention targets with images, proprioception, and actions. Its reported collection contains 12,000 demonstrations across 40 tasks; gaze is propagated between calibrated views to supervise attention during training, rather than required during deployment. This is robot-view teleoperation supervision, not an additional human egocentric corpus. Its collection scale also does not establish public availability of the full dataset, which was not verified in the checked release sources.



\begin{table}[!t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.15}
\caption{\textbf{Statistics and key properties of real-robot manipulation datasets.} ``Embod.'' denotes the number of distinct embodiment types; ``Calib.'' denotes calibrated camera extrinsics. ``Dex.'' denotes dexterous-hand data. ``Anno.'' denotes subtask labels within episodes; ``Mobile'' denotes mobile manipulation data. In the ``Arm'' column, `S', `D', `H' denote single-arm, dual-arm, and Humanoid embodiments.}
\vspace{-0.2cm}
\label{tab:real-robot-datasets}
\rowcolors{2}{white}{w_blue!7}
\begin{tabular}{@{}
>{\raggedright\arraybackslash}m{0.21\textwidth}
>{\centering\arraybackslash}m{0.03\textwidth}
>{\centering\arraybackslash}m{0.035\textwidth}
>{\centering\arraybackslash}m{0.035\textwidth}
>{\centering\arraybackslash}m{0.113\textwidth}
>{\centering\arraybackslash}m{0.04\textwidth}
% >{\raggedright\arraybackslash}m{0.040\textwidth}
>{\centering\arraybackslash}m{0.33\textwidth}
>{\centering\arraybackslash}m{0.03\textwidth}
>{\centering\arraybackslash}m{0.03\textwidth}
>{\centering\arraybackslash}m{0.03\textwidth}
>{\centering\arraybackslash}m{0.04\textwidth}
@{}}
\toprule
\textbf{Dataset} & \textbf{Time} & \textbf{Arm} & \textbf{Embod.} & \textbf{Traj. / Hours} & \textbf{Tasks} & \textbf{Modality} &  \textbf{Calib.} & \textbf{Dex.} & \textbf{Anno.} &  \textbf{Mobile}  \\
\midrule\midrule
Pinto and Gupta~\cite{pinto2016supersizing} & 2015 & S & 1 & 50K / 700 & 1 & RGB; Proprio.; Act.; Grasp Succ. & \ding{55} & \ding{55} & \ding{55}  & \ding{55} \\
DAML~\cite{yu2018one} & 2018 & S & 2 & 2.9K / 4.08 & 3 & RGB; Proprio.; Act. &  \ding{55} & \ding{55} & \ding{55} & \ding{55}   \\
MIME~\cite{sharma2018multiple} & 2018 & S/D & 1 & 8.3K / 13.7 & 20 & RGB-D; Proprio.  &  \ding{55} & \ding{55} & \ding{55} & \ding{55}    \\
QT-Opt~\cite{kalashnikov2018scalable} & 2018 & S & 1 & 580k / 800 & 1 & RGB; Proprio.; Act.; Grasp Succ. & \ding{55} & \ding{55} & \ding{55} & \ding{55}  \\
RoboTurk~\cite{mandlekar2018roboturk} & 2018 & S & 3 & 2.1K / 111.3 & 3 & RGB-D; Proprio.; &  \ding{55} & \ding{55} & \ding{55} &  \ding{55}  \\
RoboNet~\cite{dasari2020robonet} & 2019 & S & 7 & 162k / 833.3 & - & RGB; Proprio.; Act. &  \ding{55} & \ding{55} & \ding{55} &  \ding{55}   \\
MT-Opt~\cite{kalashnikov2021mt} & 2021 & S & 1 & 800k / - & 12  & RGB; Proprio.; Act. &  \ding{55} & \ding{55} & \ding{55} &  \ding{55}   \\
BridgeData~\cite{ebert2021bridge} & 2021 & S & 1 & 7.2k / - & 71 &  RGB; Proprio.; Act. & \ding{55} & \ding{55} & \ding{55} &  \ding{55}   \\
BC-Z~\cite{jang2022bc} & 2022 & S & 1 & 26K / 125 & 100 & RGB; Proprio.; Act.; Lang. & \ding{55} & \ding{55} &  \ding{55} & \ding{55}  \\
RT-1~\cite{brohan2022rt} & 2022 & S & 1 & 130K / - & 700+ & RGB; Proprio.; Act.; Lang. & \ding{55} & \ding{55} &  \ding{55} & \ding{51}  \\
FurnitureBench~\cite{heo2025furniturebench} & 2023 & S & 1 & 5.1K / 219.6 & 9 & RGB-D; Proprio.; Act. & \ding{55} & \ding{55} & \ding{55} &  \ding{55}  \\
RH20T~\cite{fang2023rh20t} & 2023 & S & 4 & 110K / - & 147  & RGB-D; Proprio.; Act.; Lang.; Tactile; Force; Audio & \ding{51} & \ding{55} & \ding{55}  & \ding{55} \\
RoboSet~\cite{bharadhwaj2024roboagent} & 2023 & S & 1 & 98.5K / - & 48  & RGB-D; Proprio.; Act.; Lang.; Force; Torque & \ding{55} & \ding{51} & \ding{51} &  \ding{55}  \\
BridgeData V2~\cite{walke2023bridgedata} & 2023 & S & 1 & 60.1K / - & 13 & RGB; Proprio.; Act.; Lang. & \ding{55} & \ding{55} & \ding{55} & \ding{55}  \\
% Aloha (Optional)~\cite{zhao2023learning} & 2023 & Dual & 1 & 300 / - & 6  & RGB; Proprio.; Act. & \ding{55} & \ding{55} & \ding{55} &  \ding{55}  \\
Open X-Embodiment~\cite{o2024open} & 2023 & S/D & 22 & 2.4M / - & 527 & RGB-D; Proprio.; Act.; Lang.; Force &  \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
% Mobile-Aloha (Optional)~\cite{fu2024mobile} & 2024 & Dual & 1 & 276 / - & 5  & RGB; Proprio.; Act. & \ding{55} & \ding{55} &  \ding{55} & \ding{51} \\
ALOHA Unleashed~\cite{zhao2024aloha} & 2024 & D & 1 & 26.2K / - & 5  & RGB; Proprio.; Act. & \ding{55} & \ding{55} & \ding{55} & \ding{55}  \\
% OmniH2O (Optional)~\cite{he2024omnih2o} & 2024 & Humanoid & 1 & - / 0.67 & 6 & RGB; Proprio.; Act. & \ding{55} & \ding{51} & \ding{55} & \ding{51} \\
% HumanPlus (Optional)~\cite{fu2024humanplus} & 2024 & Humanoid & 1 & 240 / - & 6 & RGB; Proprio.; Act. & \ding{55} & \ding{51} & \ding{55} & \ding{51}  \\
% BRMData (Optional)~\cite{zhang2024empowering} & 2024 & Dual & 4 & 0.5k / - & 10 & RGB-D; Proprio.; Act.; Lang.; Torque & \ding{55} & \ding{55} & \ding{55} & \ding{51} \\
DROID~\cite{khazatsky2024droid} & 2024 & S & 1 & 76K / 350 & 86 & RGB; Proprio.; Act.; Lang. & \ding{51} & \ding{55} & \ding{55} & \ding{55} \\
EgoMimic~\cite{kareer2025egomimic} & 2024 & D & 1 & 1K / 12 & 3 & RGB; Proprio.; Act. & \ding{51} & \ding{55} & \ding{55} & \ding{55}\\
FMB dataset~\cite{luo2025fmb} & 2024 & S & 1 & 22.6K / - & 2 & RGB-D; Proprio.; Act.; Force; Torque & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
RoboMIND~\cite{robomind2025} & 2024 & S/D & 4 & 107K / 305.5 & 479 & RGB; Proprio.; Act.; Lang.; Fail. labels & \ding{51} & \ding{51} & \ding{51} & \ding{55} \\
AgiBot World Beta~\cite{bu2025agibot} & 2025 & D & 1 & 1M / 2976.4 & 217 & RGB-D; Proprio.; Act.; Lang.; Force & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
REASSEMBLE~\cite{sliwowski2025reassemble} & 2025 & S & 1 & 4.6K / 13.02 & 121 & RGB; Proprio.; Act.; Audio; Force; Torque & \ding{51} & \ding{55} & \ding{51} & \ding{55} \\
PH2D~\cite{qiu2025humanoid} & 2025 & H & 1 & 1.6K /  -  & - & RGB; Proprio.; Act.; Lang. & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\
AIST-Bimanual~\cite{aist2025bimanip} & 2025 & D & 1 & 10.7K / - & 119 & RGB; Proprio.; Act.; Lang. & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
ActionNet~\cite{fourier2025actionnet} & 2025 & H & 3 & 30K / 140 & - & RGB-D; Proprio.; Act.; Lang. & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\
MotionTrans~\cite{yuan2025motiontrans} & 2025 & S & 1 & 1.5K / -  & 15 & RGB; Proprio.; Act.; Lang. & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\
Open Galaxea~\cite{jiang2025galaxea} & 2025 & D & 1 & 20.5K / 500 & 150 & RGB-D; Proprio.; Act.; Lang. & \ding{55} & \ding{55} & \ding{51} & \ding{51} \\
RealSource World~\cite{realsourceworld} & 2025 & D & 1 & 26.7K / - & 35 & RGB; Proprio.; Act.; Lang.; Force; Torque &  \ding{51} & \ding{55} & \ding{51} & \ding{55} \\
RoboCOIN~\cite{wu2025robocoin} & 2025 & D & 15 & 180K / - & 421 & RGB-D; Proprio.; Act.; Lang. & \ding{55} & \ding{51} & \ding{51} & \ding{55} \\
% BEAVR Bot datasets (Optional)~\cite{posadas2025beavr} & 2025 & Single & 1 & 101 / - & 6 & RGB; Proprio.; Act. &  \ding{55} & \ding{51} & \ding{55} & \ding{55} \\
Humanoid Everyday~\cite{zhao2025humanoid} & 2025 & H & 2 & 10.3k / 27.8+  & 260 & RGB-D; Proprio.; Lang.; Tactile; LiDAR; IMU; Odometry & \ding{55} & \ding{51} & \ding{55} & \ding{51} \\
RoboMIND 2.0~\cite{hou2025robomind} & 2026 & S/D & 6 & 310K / 1000+  & 739 & RGB-D; Proprio.; Act.; Lang.; Tactile; Force; Torque; Fail. labels &  \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
DECO-50~\cite{li2026deco} & 2026 & D & 1 & 8K / 50+ & 28  & RGB; Proprio.; Act.; Tactile & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\
Dexora~\cite{zhang2026dexora} & 2026 & D & 1 & 12.2K / 40.5 & 200 & RGB; Proprio.; Act.; Lang. & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\
MolmoAct2-BimanualYAM~\cite{fang2026molmoact2} & 2026 & D & 1 & 34.5K / 720 & 736 & RGB; Proprio.; Act.; Lang. & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
MolmoAct2-SO100/101~\cite{fang2026molmoact2} & 2026 & S & 2 & 38K / 184 & 1315  & RGB; Proprio.; Act.; Lang. & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
AgiBot World 2026~\cite{agibotworld2026} & 2026 & D & 1 & 20.7K / - & - & RGB-D; Proprio.; Act.; Lang.; Tactile & \ding{51} & \ding{51} & \ding{51} & \ding{51}  \\
Unitree UnifoLM-WBT~\cite{unitree2026unifolm} & 2026 & H & 1 & 4.5K / 30.74 & 14 & RGB; Proprio.; Act.; Lang. & \ding{55} & \ding{51} & \ding{55} & \ding{51}  \\
Open-H-Embodiment~\cite{nelson2026open} & 2026 & S/D & 20 & 125.8K / 780 & 33 & RGB; Proprio.; Lang. &  \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
Baihu-VTouch~\cite{hua2026vtouch++} & 2026 & S/D & 3 & - / 1000+ & 380+ & RGB-D; Proprio.; Act.; Lang.; Tactile & \ding{55} & \ding{51} & \ding{55} & \ding{51} \\
LET-Base-Dataset~\cite{lejurobotics2026letbase} & 2026 & H & 2 & 91.5K / 1000+ & 31 & RGB-D; Proprio.; Lang.; IMU & \ding{55} & \ding{51} & \ding{51} & \ding{55} \\
LET-Dex-Dataset & 2026 & H & 1 & 3K / 20 & 14 & RGB-D; Proprio.; Lang.; Tactile; Force; Torque; IMU & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\
% LET-Body-Dataset & 2026 & H & 1 & - / - & 20+ & RGB-D; Proprio.; Lang.; IMU & \ding{55} & \ding{51} & \ding{55} & \ding{51} \\
% RoVid-X~\cite{deng2026rethinking} & 2026 & Single+Dual & Multiple & 4M / 10k+ & 1300+ & RGB-D; Opticflow &\ding{55} & \ding{51} & \ding{55} & \ding{55} \\
% LingBot-Depth Dataset~\cite{tan2026masked} & 2026 & Single & 2 & 581K / - & - & RGB-D & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
Haptile~\cite{alian2026haptile} & 2026 & S & 1 & 1.7K / 12.5 & 38 & RGB; Proprio.; Act.; Lang.; Tactile & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
% DexScale (unreleased) & 2026 & Dual & 2 & 10w / - & 300 & RGB-D; Proprio.; Act.; Lang. & \ding{55} & \ding{51} & \ding{55} & \ding{55}  \\
OmniViTac~\cite{zheng2026omnivta} & 2026 & S & 1 & 21.9K / - & 86 & RGB-D; Proprio.; Act.; Lang.; Tactile & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
ABC-130K~\cite{abc2026} & 2026 & D & 1 & 130.7K / 3591 & 197 & RGB; Proprio.; Act.; Lang.; Torque & \ding{55} & \ding{55} & \ding{51} & \ding{55} \\
\bottomrule
\end{tabular}%
\end{table}



\subsection{Embodiment and Modalities}
Real-robot datasets vary substantially in the physical embodiments through which interaction data are collected. Early datasets were predominantly built around fixed-base, single-arm manipulators equipped with parallel grippers, as exemplified by large-scale grasping and manipulation datasets such as Pinto and Gupta, QT-Opt, and RoboNet~\cite{pinto2016supersizing,kalashnikov2018scalable,dasari2020robonet}. This configuration offers a relatively constrained action space and facilitates scalable data collection, but covers only a limited range of whole-body and coordinated manipulation behaviors. Later datasets increasingly incorporate dual-arm systems for coordinated and bimanual manipulation~\cite{zhao2023learning,zhao2024aloha,aist2025bimanip}, mobile manipulators that jointly control the base and upper body~\cite{fu2024mobile,jiang2025galaxea}, and humanoid platforms involving whole-body motion and locomotion~\cite{he2024omnih2o,fu2024humanplus,zhao2025humanoid}. More recent efforts further extend data collection to dexterous hands and heterogeneous robot fleets, enabling the study of fine-grained contact-rich manipulation and cross-embodiment learning~\cite{wu2025robocoin,hou2025robomind,zhang2026dexora}.

Another notable trend is the increasing richness of sensing modalities in real-robot datasets. Beyond the standard vision-proprioception-action interface, several datasets incorporate additional signals to capture aspects of physical interaction that cannot be reliably inferred from images alone. Tactile sensing has emerged as an important complementary modality for contact-rich and dexterous manipulation, as it provides local, surface-level information about contact location, pressure distribution, incipient slip, grasp stability, and object-hand interaction states~\cite{fang2023rh20t,zhao2025humanoid,hou2025robomind,li2026deco,zheng2026omnivta,alian2026haptile,yu2026prism}. Recent datasets increasingly treat tactile sensing as a first-class evaluation signal rather than an auxiliary channel: SoftVTBench~\cite{jing2026softvtbench} synchronizes dual-finger tactile images and marker motion at 20\,Hz with independent finite-element ground truth, allowing slip and excessive compression to be measured even when a task nominally succeeds. In contrast, force and torque measurements typically characterize the net interaction wrench at the wrist, gripper, or robot joints, offering a more global view of contact forces and interaction dynamics~\cite{fang2023rh20t,sliwowski2025reassemble,luo2025fmb,yu2026prism}. Audio can further provide complementary cues about collisions, friction, and task progression~\cite{fang2023rh20t,sliwowski2025reassemble}. Whole-body platforms may additionally include IMU, LiDAR, and odometry signals to represent balance, locomotion, and spatial navigation~\cite{zhao2025humanoid,lejurobotics2026letbase}. These richer multimodal observations not only enable a more comprehensive characterization of robot and environment interaction, but also increase heterogeneity across datasets.

Proprioceptive and action representations also differ considerably across embodiments. Fixed-base manipulators commonly record joint positions (qpos), represented as an ordered vector of joint coordinates, or end-effector (EEF) poses, represented by the Cartesian position and orientation of the wrist or tool, together with gripper states. Correspondingly, actions are typically expressed in either joint space or Cartesian EEF space~\cite{dasari2020robonet,ebert2021bridge,heo2025furniturebench,bharadhwaj2024roboagent,fang2023rh20t,o2024open}. Dexterous hands, due to their high-dimensional articulated structures, are typically represented through finger joint positions~\cite{robomind2025,wu2025robocoin,li2026deco,zhang2026dexora}, sometimes complemented by fingertip poses to facilitate alignment with human data~\cite{yang2025egovla,fu2025metis,zheng2026egoscale}. Mobile and humanoid platforms further incorporate base velocity, torso configuration, and whole-body joint states~\cite{fu2024mobile,zhao2025humanoid,hou2025robomind,unitree2026unifolm}.

These differences affect not only the dimensionality of the learning problem, but also the extent to which data can be shared across platforms. Joint-space representations provide direct and precise control for articulated hands, but are strongly tied to robot morphology. In contrast, end-effector-centric representations can offer a more transferable interface for arm motion across embodiments, although they still require consistent coordinate frames and control conventions. In policy learning, proprioceptive states and actions are often normalized to maintain suitable numerical scales and facilitate learning across embodiments. Common choices include MinMax, Q01-Q99, and MeanStd normalization~\cite{wu2026foundationapplicationimprovingvla}.


\subsection{Data Collection Paradigms}
\subsubsection{Script}
Scripted collection broadly refers to data-generation processes in which robot behavior is executed without continuous human control. Rather than manually controlling each episode, human effort is shifted toward designing the task logic, control pipeline, and execution conditions. This separation between system design and episode-level execution enables repeated and parallel data collection at relatively low marginal cost. Depending on how robot actions are produced, scripted collection can be broadly categorized into rule-based execution, trajectory playback, and autonomous policy rollouts.

\noindent\textbf{Rule-Based Execution.}
In rule-based collection, robot behavior is generated through manually specified task logic, often implemented as action sequences, finite-state machines, or heuristic controllers. A task is typically decomposed into predefined stages, such as detecting a target, selecting an interaction pose, approaching the target, executing the grasp, and transporting the object to a designated region. Within this pipeline, inverse kinematics, motion planning, and trajectory optimization can be used to convert stage-level goals into kinematically feasible and collision-free robot motions, while visual observations or sensor thresholds determine target poses and trigger transitions between stages. Early large-scale grasping datasets adopted such structured pipelines to execute repeated grasp attempts and automatically record both successful and failed interactions~\cite{pinto2016supersizing,dasari2020robonet,wang2025fieldgen}. Rule-based execution is particularly effective for tasks with clearly specified objectives, structured workspaces, and reliable reset mechanisms. However, because both the task decomposition and motion-generation process rely on predefined assumptions, the collected behaviors may exhibit limited diversity and may not generalize well to unanticipated states or complex contact interactions.

\noindent\textbf{Trajectory Playback.}
Trajectory playback collects data by re-executing previously recorded robot motions. The source trajectories may originate from human teleoperation, kinesthetic teaching, motion planning or earlier policy rollouts. During playback, the robot can reproduce demonstrations under different object configurations or environmental conditions, and perturbations may be introduced into the initial state, trajectory, or control parameters to increase variation. This approach reduces the need for repeated human operation while preserving the overall structure of successful demonstrations. For example, RoboSet combines human-collected demonstrations with playback-based execution to expand its real-robot experience~\cite{bharadhwaj2024roboagent}. Nevertheless, playback is sensitive to discrepancies between the original and current environment, since open-loop reproduction may fail when object locations or contact conditions change substantially. Closed-loop correction and replanning are therefore often required for reliable reuse.

\noindent\textbf{Autonomous Policy Rollouts.}
A more adaptive form of automated collection uses learned or heuristic policies to interact with the environment and generate new trajectories. Such policies may be obtained through reinforcement learning, imitation learning, or prior rounds of data collection, and can be iteratively improved as additional experience becomes available. Large-scale systems such as QT-Opt~\cite{kalashnikov2018scalable} and MT-Opt~\cite{kalashnikov2021mt} use autonomous rollouts to collect interaction data across repeated task executions, enabling the dataset and policy to improve through a continual data-generation cycle. RoboSet~\cite{bharadhwaj2024roboagent} similarly includes heuristic policy rollouts alongside human demonstrations and trajectory playback. Compared with fixed scripts, autonomous rollouts can respond to observations and cover a broader range of states, including policy failures and recovery behaviors. However, their data distribution is strongly shaped by the capabilities and exploration strategy of the current policy, potentially reinforcing existing biases or producing large quantities of low-quality trajectories.

\subsubsection{Teleoperation}
Teleoperation collects robot demonstrations by allowing a human operator to continuously control the robot during task execution. Relative to scripted collection, it can more naturally capture adaptive, goal-directed, and contact-rich behaviors, particularly in tasks where suitable control policies are not yet available. As illustrated in Figure~\ref{fig:umi_real_robot}, teleoperation systems exhibit diverse configurations.

\noindent\textbf{Kinesthetic Teaching.}
Kinesthetic teaching provides the most direct form of human control: the operator physically guides the robot arm or end effector through the desired motion while the system records joint states, end-effector poses, and gripper commands. This approach requires little additional interface hardware and allows operators to specify precise trajectories through direct physical interaction, as demonstrated in datasets such as MIME~\cite{sharma2018multiple}. It is particularly suitable for fixed-base manipulators and tasks requiring accurate geometric guidance. However, physical manipulation of the robot can impose substantial operator effort, and the approach is difficult to apply to high-payload systems, mobile platforms, or complex whole-body embodiments. HALO~\cite{yang2026halocollection} extends kinesthetic teaching to coordinated mobile manipulation by coupling direct guidance of the arms with a passive collection platform and aligning its recorded motion to the powered base used at deployment.

\noindent\textbf{Leader-Follower Teleoperation.}
Leader-follower systems use a dedicated input mechanism whose motion is mapped to a follower robot. When the leader and follower have identical or closely matched kinematic structures, joint-level correspondence provides an intuitive and precise control interface. This paradigm has been widely adopted for bimanual manipulation, as exemplified by ALOHA and its subsequent extensions~\cite{zhao2023learning,zhao2024aloha}, as well as larger bimanual datasets such as AIST-Bimanual~\cite{aist2025bimanip} and Open Galaxea~\cite{jiang2025galaxea}. GELLO~\cite{wu2024gello} further demonstrates that the leader can be implemented as a low-cost, scaled, and kinematically equivalent replica of the target arm, using 3D-printed components and inexpensive actuators while retaining direct joint-level correspondence. Leader-follower control is well suited to coordinated two-arm behaviors because it preserves temporal synchronization between both arms and reduces the complexity of Cartesian control. Its main limitation is the dependence on specialized, and often embodiment-specific, hardware, which can constrain portability across robot platforms.

\noindent\textbf{Integrated Leader-Follower Teleoperation.}
Integrated leader-follower teleoperation combines the input device and controlled robot within the same mechanism: the operator steers a gravity-compensated arm through an end-effector handle while the system records robot states, visual observations, and interaction signals. This method provides direct visual and force feedback, supports precise contact-rich manipulation, and avoids the kinematic-mapping errors of separate leader arms. Eliminating the dedicated leader device also reduces hardware, calibration, and workspace requirements. A representative practical example is the ARX AC-One, which has recently been used as a real-world platform for bimanual manipulation research~\cite{bi2025motusunifiedlatentaction,cai2026internvla}. The main drawback is that the operator's hand may appear in training images but be absent during autonomous deployment, creating a visual distribution shift. However, existing evidence from human-to-robot~\cite{yang2025egovla,zheng2026egoscale} transfer suggests that models can learn to accommodate such differences during pretraining.

\noindent\textbf{Device-Mediated Teleoperation.}
A more portable alternative uses generic input devices, including VR or XR controllers, smartphones, SpaceMouse devices and joysticks. Human inputs are commonly interpreted as Cartesian end-effector poses or velocities and converted into robot joint commands through inverse kinematics or low-level controllers. RoboTurk~\cite{mandlekar2018roboturk}, for example, uses a mobile device for six-degree-of-freedom control, while DROID~\cite{khazatsky2024droid} employs VR controllers to collect manipulation demonstrations across diverse environments. SpaceMouse and haptic devices have also been used in datasets such as FMB~\cite{luo2025fmb} and REASSEMBLE~\cite{sliwowski2025reassemble}. Touchscreens provide an even lower-cost channel for planar tasks: a recent learning-from-demonstration dataset records 3,142 handwriting demonstrations from 22 participants across all 52 Latin character-case combinations through a touchscreen teleoperation interface, capturing planar position, contact force, and timing~\cite{kenan2026robot}. For mobile manipulators, foot pedals can provide an additional hands-free control channel for commanding base motion, allowing the operator to navigate the platform while keeping both hands available for arm manipulation. Because these devices are largely independent of robot morphology, they can be deployed across different manipulators with relatively limited hardware modification. Yet their indirect control interfaces may introduce latency, scaling ambiguities, and reduced precision, especially for coordinated, high-dimensional, or contact-intensive tasks. A recent trend is to push this hardware independence from the input device to the whole collection rig: ModPack~\cite{citron2026modpack} packages computation, power, communication, and storage into a self-contained wearable backpack and exposes plug-and-play capability modules for joint-level teleoperation with haptic feedback, mobile manipulation, and active perception, so that the same interface can be reused across robot platforms and task domains.

\noindent\textbf{Vision-Based Teleoperation.}
Vision-based systems infer human body, arm, or hand motion directly from RGB or RGB-D observations, without requiring physical markers or dedicated wearable sensors. The estimated poses are then retargeted to the robot while accounting for kinematic feasibility and joint constraints. Such approaches can support both whole-body humanoid control and dexterous-hand teleoperation. HumanPlus~\cite{fu2024humanplus}, for example, transfers monocularly estimated human motion to a humanoid robot, while DexPilot~\cite{handa2020dexpilot} and Anyteleop~\cite{qin2023anyteleop} map visually estimated human hand motion to a dexterous robot hand. By reducing the need for specialized sensing hardware, vision-based teleoperation provides a low-cost and accessible interface, although its performance remains sensitive to occlusion, fast motion, and pose-estimation errors.

\noindent\textbf{Wearable and Motion-Capture Retargeting.}
Wearable systems capture human motion using devices such as inertial suits, optical trackers, data gloves, or arm and hand exoskeletons. These interfaces can provide higher-dimensional and more stable motion measurements than generic controllers, making them particularly suitable for bimanual, dexterous, and whole-body teleoperation. RoboMIND~\cite{robomind2025,hou2025robomind} combines multiple teleoperation interfaces, including motion-capture systems, to collect data across heterogeneous robot embodiments, while RoboCOIN~\cite{wu2025robocoin} extends wearable control to a large collection of dual-arm platforms. For dexterous manipulation, systems such as Dexora~\cite{zhang2026dexora} use arm exoskeletons and VR-based hand control to capture coordinated arm and finger motion. Whole-body teleoperation systems further map human upper-body, locomotion, and base motion to humanoid robots~\cite{unitree2026unifolm,zhao2025humanoid}, and comparable interfaces have been built for wheeled bimanual platforms, where a single VR interface coordinates base and dual-arm control to collect multimodal mobile-manipulation demonstrations~\cite{yang2026learning}. The required mapping depends on the sensing interface and the degree of correspondence between the human and robot embodiments. Exoskeleton-based systems often provide direct joint-level control, whereas data gloves and motion-capture devices typically require calibration and kinematic retargeting to account for differences in scale, joint ranges, and morphology. Glove-based sensing introduces a further, less obvious source of error: because the tactile elements must remain soft and flexible to preserve hand dexterity, they respond not only to contact force but also to hand pose, producing pose-related artifacts that raise the minimum detectable force and cause missed or late contact onsets in the low-force range. A glove-agnostic pose-aware framework~\cite{yu2026poseaware} characterizes these artifacts and mitigates them algorithmically by conditioning force estimation on hand pose, without modifying the glove, which is relevant to any pipeline that treats glove readings as contact ground truth.

\noindent\textbf{Feedback Mechanisms.} Feedback mechanisms constitute another important dimension of teleoperation-system design. Visual feedback provides the operator with observations of the environment, objects, and robot state through external or egocentric cameras. Immersive systems further employ stereoscopic displays and head-tracked active viewpoints to improve depth perception and spatial awareness~\cite{cheng2024open,ding2025bunny}. Force feedback transmits interaction forces or end-effector resistance from the robot to the operator through bilateral leader devices, haptic controllers, or exoskeletons, enabling more precise regulation of contact during insertion, assembly, and other force-sensitive tasks~\cite{sliwowski2025reassemble,zhang2025doglove}. Tactile feedback communicates localized contact events at the fingers or grasp interface, for example, through vibration, pressure, or fingertip stimulation, helping the operator perceive contact onset and adjust grasping behavior~\cite{ding2025bunny,zhang2025doglove,alian2026haptile}. The integration of these feedback channels improves teleoperation accuracy, stability, and operator awareness, enabling more natural control and higher-quality demonstrations, particularly in contact-rich tasks. A complementary direction moves in the opposite direction along the same loop, using the robot to assist the operator: goal-free intent-inference frameworks estimate which object or grasp region the operator is reaching for from partial motion, and can then bias assistance toward feasible grasps. GUIDER~\cite{kenny2026guider} evaluates such a framework on recorded real-robot manipulation data under the original temporal conditions, reporting a mean time to confident prediction of 3.7\,s and 96.4\% prediction stability across 20 manipulation steps. Shared-autonomy mechanisms of this kind can lower operator burden during long collection sessions, but they also shape the recorded trajectories, so the degree of assistance is itself a dataset property worth reporting.

\subsubsection{Human-in-the-Loop Enhancement}
Human-in-the-loop enhancement is an iterative real-robot data collection paradigm in which a human supervisor intervenes during policy execution and records corrective actions at difficult or failure-prone states. Rather than repeatedly collecting complete demonstrations, it selectively augments the dataset with policy-induced states, failure cases, and recovery trajectories that are underrepresented in the original training data.

Following the dataset-aggregation principle introduced by DAgger~\cite{ross2011reduction}, robot-learning methods have progressively improved the efficiency and scalability of this process. Intervention Weighted Regression~\cite{mandlekar2020human} collects corrective demonstrations through remote teleoperation and increases their contribution during training. ThriftyDAgger~\cite{hoque2021thriftydagger} selectively requests assistance according to state novelty and estimated failure risk, while Sirius~\cite{liu2025robot} continuously incorporates intervention data gathered during robot deployment. Fleet-DAgger~\cite{hoque2023fleet} extends this collection process to multiple concurrently operating robots. In dexterous manipulation, DexCap~\cite{wang2024dexcap} records human takeovers and residual corrections during policy rollouts. IntervenGen~\cite{hoque2024intervengen} subsequently improves data efficiency by generating additional corrective trajectories from a small number of human interventions. More recently, CR-DAgger~\cite{xu2026compliant} collects compliant delta-action corrections for contact-rich manipulation without fully interrupting autonomous execution. Overall, human-in-the-loop enhancement transforms errors encountered during real-robot deployment into targeted training data, improving the coverage of challenging states while reducing the need for full-trajectory demonstrations.

PrimeBot household data~\cite{xu2026scalingbimanual} illustrates the complementarity of expert demonstrations and deployment-time corrections. The collected corpus combines 531.7 hours of physical robot teleoperation with approximately 1,000 hours of bimanual UMI demonstrations, while the public release contains the real-robot data and staged UMI subsets. Clothes-folding experiments show diminishing returns from additional expert data and continued improvements from human interventions at policy-induced failure states, supporting targeted corrective collection rather than an unrestricted scaling claim.


SharpaDex v1.0~\cite{sharpadex_v1_2026} extends bimanual teleoperation toward fingertip-tactile supervision, pairing multi-view RGB with robot states, commands, tactile force/torque and tactile video, and temporally aligned language. Its official release reports 28,993 demonstrations across 59 tasks under CC BY-NC 4.0; the LeRobot v2.1 and v3.0 exports represent the same demonstrations and must not be counted twice.

\subsection{Scale and Diversity}
The scale of real-robot data has increased substantially over the past decade. Early datasets often accumulated large numbers of interactions within a narrowly defined task distribution. For example, Pinto and Gupta~\cite{pinto2016supersizing} and QT-Opt~\cite{kalashnikov2018scalable} collected tens or hundreds of thousands of grasping trials, but primarily focused on a single behavior. Subsequent efforts expanded both the number of trajectories and the breadth of tasks. MT-Opt~\cite{kalashnikov2021mt} contains approximately 800K episodes across 12 tasks, while RT-1~\cite{brohan2022rt} and RoboMIND~\cite{robomind2025} cover hundreds of manipulation skills with 130K and 107K trajectories, respectively. More recent datasets have reached million-scale collection or thousands of hours of interaction. AgiBot World Beta~\cite{bu2025agibot} reports one million trajectories and nearly 3,000 hours of data, while RoboMIND 2.0~\cite{hou2025robomind} contains more than 310K trajectories across 739 tasks and over 1,000 hours of execution. Cross-dataset initiatives such as Open X-Embodiment~\cite{o2024open} further aggregate more than two million trajectories from multiple institutions and robot platforms. The ArmnetBench rollout release~\cite{selvaraj2026rollout} illustrates a complementary source of diversity: it publishes 600 teleoperated demonstrations and 3,118 outcome-labelled policy rollouts on the same 12 tabletop tasks, including 2,288 failures.

For policy learning, data diversity is often more consequential than the raw number of trajectories, as it determines the range of states, behaviors, and interaction conditions represented during training. A clear trend in recent real-robot datasets is therefore the expansion of task coverage, from narrowly defined behaviors such as grasping or assembly to hundreds of household, industrial, mobile-manipulation, and dexterous tasks~\cite{wu2025robocoin,hou2025robomind,fang2026molmoact2,zhang2026dexora}. Task diversity alone, however, does not guarantee coverage of the interaction regimes a policy will face. Datasets remain concentrated on short-horizon, low-contact behaviors such as pick-and-place, which underrepresent the precision control and force or tactile regulation required by industrial assembly~\cite{yu2026prism}, and evaluation that reports only task success can hide whether a policy achieved that success while slipping or over-compressing the object~\cite{jing2026softvtbench}. Coverage should therefore be assessed along contact and precision axes as well as task counts. This task diversity is accompanied by increasing variation in objects, scene layouts, initial configurations and camera viewpoints, providing broader coverage of the state distributions encountered at deployment. At the same time, datasets increasingly span heterogeneous embodiments, including single-arm and bimanual manipulators, mobile platforms, humanoids, and dexterous hands, as well as richer sensing modalities such as RGB-D, force and torque, audio, IMU, LiDAR, and odometry~\cite{o2024open,wu2025robocoin,zhao2025humanoid,hou2025robomind}. Together, diversity across tasks, environments, embodiments, and modalities provides the foundation for learning policies that are more robust and transferable beyond a narrowly defined data-collection setting.


Beyond task, embodiment, and modality diversity, trajectory-level diversity captures variations in how the same nominal task is executed across demonstrations. Such variation may arise from differences in initial and terminal states, motion paths, contact sequences, and execution speeds, thereby broadening the state-action distribution covered within each task. The Cartesian distributions of keyframes in Figure~\ref{fig:diversity} provide an intuitive illustration of the resulting differences in spatial coverage and distributional structure. In the examples shown, AgiBot-World-2026~\cite{agibotworld2026} exhibits several well-separated spatial clusters, suggesting coverage of distinct workspace regions and interaction heights. RoboMIND~\cite{robomind2025} shows a more compact and anisotropic distribution, whereas RoboMIND 2.0~\cite{hou2025robomind} presents broader, partially connected, and vertically stratified spatial coverage.

\subsection{Advantages and Limitations}
Real-robot data provide physically grounded supervision by directly capturing the relationship between robot observations, actions, and their physical consequences. Compared with simulation or human videos, they naturally reflect real sensing noise, control latency, contact dynamics, and hardware constraints. Moreover, the recorded actions are directly executable on the corresponding platform, making such data particularly valuable for learning reliable manipulation policies and recovery behaviors.

The main limitation is the high cost of collection. Real-robot data require physical hardware, human operation or automated collection pipelines, repeated environment resets, maintenance, and safety supervision, which restrict large-scale and parallel data acquisition. In addition, many datasets remain concentrated on specific robots, tasks, and environments. Differences in embodiment, sensor configuration, coordinate systems, and action representation further complicate data aggregation and cross-platform transfer.

\begin{wbtakeaway}
\bReal~\textbf{Real-robot data} sits at the apex: it provides direct robot control signals together with observations of physical interactions between the robot and the real world. We believe that future real-robot data development should proceed along three directions. First, teleoperation systems should support simpler, smoother, and more intuitive control while preserving fine-grained trajectories and direct physical interaction feedback. In this respect, \emph{Integrated Leader-Follower Teleoperation} provides a promising direction because of its relatively low hardware cost, ease of use, and capacity for fluent demonstration collection. Second, real-robot datasets should capture broader in-the-wild variations in scenes, objects, and environmental conditions. AIGC may complement physical collection by synthesizing embodiment-specific data or augmenting scenes and observations, thereby expanding environmental diversity without requiring proportional increases in real-world deployment. Third, data collection should extend beyond human teleoperation to include policy rollouts, which reflect how an embodied agent explores the physical world under its own induced state distribution. Human-in-the-loop interventions during these rollouts can further transform failures into recovery trajectories, providing supervision for error correction, task continuation, and improved policy robustness.
\end{wbtakeaway}

